Constraints on future analysis metadata systems in High Energy Physics

In High Energy Physics (HEP), analysis metadata comes in many forms -- from theoretical cross-sections, to calibration corrections, to details about file processing. Correctly applying metadata is a crucial and often time-consuming step in an analysis, but designing analysis metadata systems has historically received little direct attention. Among other considerations, an ideal metadata tool should be easy to use by new analysers, should scale to large data volumes and diverse processing paradigms, and should enable future analysis reinterpretation. This document, which is the product of community discussions organised by the HEP Software Foundation, categorises types of metadata by scope and format and gives examples of current metadata solutions. Important design considerations for metadata systems, including sociological factors, analysis preservation efforts, and technical factors, are discussed. A list of best practices and technical requirements for future analysis metadata systems is presented. These best practices could guide the development of a future cross-experimental effort for analysis metadata tools.

==> review.tex <==
page 2:


Why do longer run times of experiments mean that the analyses are larger (l 21)? This is not apparent to me. (A+S)


page 5:

(l 41)  What do you mean with matching formats? What should be matched to what? Could you give a deciated example why this is a technological challenge? (TJ)

> We have rephrased the sentence for clarification -- the challenge is to anticipate the diverse needs and address them in a sufficiently constrained range of formats, such that metadata providers have a model to follow, rather than making up a hodgepodge of formats that need to be shoehorned in, which was the experience of ATLAS/CMS with the derivation of analysis calibration information. Flexibility has to be present in the system to address novel requirements and incorporate new solutions. 

page 6:
(l 14) the sentence implies that larger collaborations do have dedicated person power for the (meta)data manangement. My experience is different. Can you explain this a bit more, e.g. related to HEP experimetns? (A - response)

(No change to the text)
> Within ATLAS and CMS, for example, there are dedicated teams who manage some of the central tools and databases where metadata is stored  (particularly metadata related to detector calibration data or the central production of Monte Carlo datasets). This of course does not cover all metadata sources, but it is at least a start. Smaller collaborations are less likely to have people with the specific expertise of setting up and maintaining databases.

page 7:
(l 35 - l 53)  In this paragraph I would like to suggest to go a little deeper into the problems of allowance of access (AAI), of (meta)data curation, and validation. Who shall be responsible for what? (?)
related to the Access Interface, I do miss a short analysis (best practice) of the current  status, the whole topic is looking to the future.(TJ)

> We have split up the paragraph to expand on the user submission discussion, and added one example from ATLAS where this was moved (from a collection of formatted text files) into a metadata database. From the meetings that gave rise to this document, this likely the most centralised procedure amongst the various experiments participating in the discussion. Further discussion of responsibility is challenging, as the details may vary depending on the contexts of different experiments, but we suggest some minimal features that would address typical errors.


In addition, I expected to have somewhere in teh paper a discussion on how FAIR the proposal is, as FAIR data management is nowadays the first premise for any concept of metadata handling. (N)


page 8:

(l 29)   ...for any future analysis metadata system....   Do you mean really any, or any in future HEP experiments? Is this applicable also to nuclear physics experiemtns, smaller experiments, astronomy observatories? (A - response)


page 9:

(l 36)  Here I was asking myself the question if the whole system should be used by the community (within the experiement, experts) only, or i it also useful or applicable for a open data sytem; i.e. can the system directly made be public via the CERN OPen Data Portal, e.g.?   (A)

No change to the text. 
> A metadata system like the one described here would facilitate analysis preservation  (as discussed in Section 2), but the question of how much should be directly made public and posted on the CERN Open Data Portal depends on the policies of each experiment and is beyond the scope of this document.


page 10:

Perhaps some of the above questions can be briefly addressed again in the summary, especially on the question of a possible generalisation of the proposal presented here. (ALL)

In addition, a brief outline of a timeline and perhaps a reference to the required person power would be useful for the general reader. (TJ -response)

> We explicitly restrict the scope of this paper to identifying the requirements on metadata system design. Definition of concrete solutions is intended to be a next step, in which these questions could concretely be addressed. We do mention the HL-LHC as a scale on which these challenges become more relevant, but in this case the burden of legacy infrastructure complicates the picture substantially.
